A modular massively parallel computing environment for three-dimensional multiresolution simulations of compressible flows

Numerical investigation of compressible flows faces two main challenges. In order to accurately describe the flow characteristics, high-resolution nonlinear numerical schemes are needed to capture discontinuities and resolve wide convective, acoustic and interfacial scale ranges. The simulation of realistic 3D problems with state-of-the-art FVM based on approximate Riemann solvers with weighted nonlinear reconstruction schemes requires the usage of HPC architectures. Efficient compression algorithms reduce computational and memory load. Fully adaptive MR algorithms with LTS have proven their potential for such applications. While modern CPU require multiple levels of parallelism to achieve peak performance, the fine grained MR mesh adaptivity results in challenging compute/communication patterns. Moreover, LTS incur for strong data dependencies which challenge a parallelization strategy. We address these challenges with a block-based MR algorithm, where arbitrary cuts in the underlying octree are possible. This allows for a parallelization on distributed-memory machines via the MPI. We obtain neighbor relations by a simple bit-logic in a modified Morton Order. The block-based concept allows for a modular setup of the source code framework in which the building blocks of the algorithm, such as the choice of the Riemann solver or the reconstruction stencil, are interchangeable without loss of parallel performance. We present the capabilities of the modular framework with a range of test cases and scaling analysis with effective resolutions beyond one billion cells using $\mathcal{O}(10^3)$ cores.

==> Inputs/Benchmarking/ParallelPerformance/neighboor_cache.tex <==
\subsubsection{Influence of Neigbor Lookup}

We have seen in \cref{algo:ComputeLoop}, that the block-based \ac{MR} scheme with \ac{ALTS} requires multiple communication routines. In theses, different communication patterns are present. Even though our neighbor-lookup routines are cheap, they need to be applied within a tree traversal. The repeated traversal is destined to potentially become a performance bottleneck. To circumvent this a cache can be utilized. As the communication patterns only change if the mesh has change, the neighbor lookup can be be done once and stored until a coarsening or refinement has been executed. We investigated if such a caching approach is favorable by running a strong and weak scaling analysis as done in \cref{sec:CurvesPerformance}. Therein, we disable the cache and hence recompute the neighbor lookup every time communication between blocks is necessary. \Cref{fig:Caches} shows the obtained speedup and runtimes for the strong and weak scaling case.

%\tikzset{external/export=false} %This shitty link to label does not compile on our shitty old work machines with externalize.
\begin{figure}
\begin{subfigure}[c]{0.5\textwidth}
\begin{center}
\begin{adjustbox}{width=\linewidth}
\begin{tikzpicture}
\begin{axis}[xmode = log, ymode = log, cycle list name = TUMcyclelist, xlabel = {Number of Ranks}, ylabel = {Speedup}]
\addplot[thick, dashed] table [x=Ranks, y=Ranks, col sep=comma, forget plot] {./ExtractedData/caches.csv};
\addplot+[thick] table [x=Ranks, y=Speedup-Strong-Std, col sep=comma] {./ExtractedData/caches.csv};
\addplot+[thick] table [x=Ranks, y=Speedup-Strong-NoCache, col sep=comma] {./ExtractedData/caches.csv};
\end{axis}
\end{tikzpicture}
\end{adjustbox}
\end{center}
\end{subfigure}
\begin{subfigure}[c]{0.5\textwidth}
\begin{center}
\begin{adjustbox}{width=\linewidth}
\begin{tikzpicture}
\begin{axis}[xmode = log, ymin = -0.1, ymax = 1.1, cycle list name = TUMcyclelist, xlabel = {Number of Ranks}, ylabel = {$\eta_w$}]
\addplot+[thick] table [x=Ranks, y=Efficiency-Weak-Std, col sep=comma] {./ExtractedData/caches.csv}; \label{plot:caches:std}
\addplot+[thick] table [x=Ranks, y=Efficiency-Weak-NoCache, col sep=comma] {./ExtractedData/caches.csv}; \label{plot:caches:no}
\end{axis}
\end{tikzpicture}
\end{adjustbox}
\end{center}
\end{subfigure}
\caption{Performance comparison with \cref{plot:caches:std} and without \cref{plot:caches:no} caching neighbor relations for strong scaling case from \cref{sec:Strongscale} and the weak scaling setup from \cref{sec:Weakscale}.}
\label{fig:Caches}
\end{figure}
%\tikzset{external/export=true}

As we can see, the performance with and with out the cache is nearly identical for small loads, \ie small number of blocks and/or small number of ranks. The higher the load the more the performance is affected. This is best visible in the weak scaling case where both the number of ranks and the number of blocks increases simultaneously. There for a Rank count of 256 the weak scaling efficiency is almost halved. With the cache in place, however, well acceptable performance is observed. We therefore kept the cache enabled in all other cases shown in this work.
